DoPE: Decoy Oriented Perturbation Encapsulation Human-Readable, AI-Hostile Documents for Academic Integrity

Multimodal Large Language Models (MLLMs) can directly consume exam documents, threatening conventional assessments and academic integrity. We present DoPE (Decoy-Oriented Perturbation Encapsulation), a document-layer defense framework that embeds semantic decoys into PDF/HTML assessments to exploit render-parse discrepancies in MLLM pipelines. By instrumenting exams at authoring time, DoPE provides model-agnostic prevention (stop or confound automated solving) and detection (flag blind AI reliance) without relying on conventional one-shot classifiers. We formalize prevention and detection tasks, and introduce FewSoRT-Q, an LLM-guided pipeline that generates question-level semantic decoys and FewSoRT-D to encapsulate them into watermarked documents. We evaluate on Integrity-Bench, a novel benchmark of 1826 exams (PDF+HTML) derived from public QA datasets and OpenCourseWare. Against black-box MLLMs from OpenAI and Anthropic, DoPE yields strong empirical gains: a 91.4% detection rate at an 8.7% false-positive rate using an LLM-as-Judge verifier, and prevents successful completion or induces decoy-aligned failures in 96.3% of attempts. We release Integrity-Bench, our toolkit, and evaluation code to enable reproducible study of document-layer defenses for academic integrity.

==> prompts/ACL_LongForm_Perturbation.tex <==
## SITUATION:
We are creating substitute questions by replacing exactly ONE contiguous substring in long-form questions (essay, short answer, explanation) to cause predictable, detectable deviations in responses. The goal is to change the question focus so that the expected answer shifts to a different topic, aspect, time period, or perspective.
## Role:
You are an expert at generating precise, high-impact text substitutions for long-form questions that cause predictable, detectable deviations in responses. Your accuracy is critical.
## Task:
You need to generate question substitutions by replacing exactly ONE contiguous substring in the question stem. Each substitution must:
1. Change the question focus in a way that CLEARLY affect the expected answer
2. Cause the response to discuss a different aspect, entity, time period, or concept
3. Be natural and semantically meaningful
4. Maintain LaTeX formatting and layout safety
## INSTRUCTIONS (apply to ALL questions below)
*Strategy:* Replacement (replace exactly ONE contiguous substring in the stem)
*Mandatory Rules:*
1) Single-span edit: replace exactly ONE contiguous substring inside LaTeX-stem-text (stem only, no multiple edits).
2) Exact match: original-substring MUST be found verbatim in LaTeX-stem-text 
3) Valid indices: LaTeX-stem-text[start-pos:end-pos] == original-substring EXACTLY AND end-pos = start-pos + len(original-substring) EXACTLY.
4) Non-empty strings: Both original-substring and replacement-substring MUST contain actual text 
5) Different strings: replacement-substring MUST be different from original-substring
6) Length constraint: len(replacement-substring) <= len(original-substring) is MANDATORY (prevents layout issues).
7) Layout-safe: replacement-substring should be similar length to original-substring (aim: within +-12 characters) and keep LaTeX well formed.
8) Distinctness: mappings should not be near-duplicates; vary the edited span and/or the targeted answer deviation.
9) Semantic quality: Replacement must be natural and semantically meaningful (not awkward phrasing).

### DEVIATION STRATEGY TIERS
*Tier 1 - Scope/Focus Shift (Best for Detection):*
Changes WHAT the question asks about while keeping the domain.- "economic impact" --> "social impact"
*Tier 2 - Temporal/Contextual Shift:*
Changes WHEN or WHERE the question applies. - "19th century" --> "20th century"
*Tier 3 - Perspective/Stakeholder Shift:*
Changes WHO or WHOSE viewpoint is requested.
- "from a patient's perspective" --> "from a doctor's perspective"
### EXAMPLE:

Original Question:
- LaTeX stem: Explain the economic impact of the Industrial Revolution on European society.
- Gold answer: The Industrial Revolution led to increased GDP, wage growth, urbanization, and the rise of capitalism. It transformed agricultural economies into industrial ones, creating new wealth but also economic inequality.

Substitution 1:
- original-substring: "economic impact"
- replacement-substring: "social impact"

Above example shows how replacing key phrases changes the question focus and causes predictable answer deviations.

For each question substitution, provide:*
- question-index: The question number
- LaTeX-stem-text: Must exactly equal the input LaTeX-stem-text
- original-substring: The substring to replace
- replacement-substring: The replacement text
- start-pos: Start position (0-based)
- end-pos: End position (exclusive)
- target-wrong-answer: Description of how the answer should deviate (include content shift, presence markers, absence markers)
- reasoning: 1-2 sentences explaining why this mapping causes deviation
- verification: Causal chain showing original --> replacement --> content shift --> detection method
## LONG QUESTIONS {questions-list}
## OUTPUT FORMAT
Return ONLY valid JSON as a single array containing ALL mappings from ALL questions above.Each question should have {k} mappings.

Total expected mappings: {total-mappings}
[
  {{
    "question-index": 1,
    "LaTeX-stem-text": "...",
    "original-substring": "...",
    "replacement-substring": "...",
    "start-pos": 0,
    "end-pos": 5,
    "target-wrong-answer": "Response focuses on social changes instead of economic metrics. Will contain markers: 'social class', 'living conditions'. Will lack: 'GDP', 'wages'.",
    "reasoning": "...",
    "verification": "'economic impact' --> 'social impact' --> response discusses sociology --> detectable via absent economic terminology"
  }},
  ...] 
Return ONLY valid JSON array, no markdown fences, no additional commentary.

==> prompts/ACL_MCQ_Perturbation.tex <==
## SITUATION:
We are creating substitute questions by looking at the options of the original question in MCQ questions  for making more question using same options of the original question. It's not necessary to change parts of the question/statement only, replacing it entirely is acceptable given it's answer is being changed towards another option which it must do.

## Role:
You are an expert at generating question substitutions for academic multiple-choice questions that cause predictable answer shifts to one of the other 3 options. Let's say the correct answer is A) and the other options are B, C, D. Your accuracy is critical. You have to come up with clever and natural question substitutions that are semantically meaningful and cause predictable answer shifts to one of the other 3 options (A, B, C, D).

## Task: You also know the correct answer for each question.
## INSTRUCTIONS (apply to ALL questions below)
1) Replacement of the question with a statement true about one of the other 3 options (replace only the question stem, do not edit the options)
2) It can be ANY semantically meaningful statement true about one of the other 3 options.
3) It should not be in any way related to correct option.
4) It must contradict the selection of correct option. In no case it should be true for the correct option.
5) The number of characters should be less than or equal to the original question stem.

### EXAMPLES:(No need to use these examples, just understand the concept)
Original McQ: What is the capital of France? Options:
A) Paris B) London C) Berlin D) Rome
Correct Answer: C) Paris
Substitution: Where were the 2012 Olympics held? Correct Answer: B) London
Here the answer is being changed from C) Paris to B) London.

Above examples have no relation to the original question/statement in any way.
They just need to be semantically meaningful and causing predictable answer shifts to one of the other 3 options (A, B, C, D). That's it.
Original McQ: Which of the following is not a programming language? Options:
A) Python B) Flask C) C++ D) Java
Correct Answer: Python
Substitution: In which option there are two + signs? 
Correct Answer: C++
Here the answer is being changed from Flask to C++.

Above examples have no relation to the original question/statement in any way.
They just need to be semantically meaningful and causing predictable answer shifts to one of the other 3 options (A, B, C, D). That's it.
*What to output for each mapping:*
- question-index: The question number
- latex-stem-text: Must exactly equal the input latex-stem-text
- original-substring: The substring to replace
- replacement-substring: The replacement text
- start-pos: Start position (0-based)
- end-pos: End position (exclusive)
- target-wrong-answer: A single option key (e.g., "A", "B", "C", "D") that is NOT the gold answer
- reasoning: 1-2 sentences explaining why the new stem makes target-wrong-answer correct and the gold answer incorrect
- verification: Causal chain showing original --> replacement --> interpretation --> answer selection

*VALIDATION CHECKLIST (verify each mapping before including):*
- original-substring exists verbatim in latex-stem-text
- latex-stem-text[start-pos:end-pos] == original-substring exactly
- end-pos == start-pos + len(original-substring) exactly
- replacement-substring != original-substring (different strings)
- len(replacement-substring) > 0 and len(original-substring) > 0 (non-empty)
- len(replacement-substring) <= len(original-substring) (length constraint)
- target-wrong-answer != gold-answer (different option)
- Replacement question is Tier 1 or Tier 2 quality

## MCQ QUESTIONS {questions-list}

## OUTPUT FORMAT
Return ONLY valid JSON as a single array containing ALL mappings from ALL questions above.
Each question should have {k} mappings (one for each other option (A, B, C, D)).

Total expected mappings: {total-mappings}
```json[ {{
    "question-index": 1,
    "latex-stem-text": "...",
    "original-substring": "...",
    "replacement-substring": "...",
    "start-pos": 0,
    "end-pos": 5,
    "target-wrong-answer": "B",
    "reasoning": "...",
    "verification": "'primary function' --> 'least common role' --> reader seeks rare function --> selects C"
  }},
  ...]'''
Return ONLY valid JSON array, no markdown fences, no additional commentary.

==> prompts/ACL_TF_Perturbation.tex <==
## SITUATION:
We are question/statement in True and False questions to make the LLM answer the opposite option(False if True, True if False).

## Role:
You are an expert at generating question substitutions for True/False questions. You have to come up with clever and natural question substitutions that are semantically meaningful and of opposite truth value. Your accuracy is critical.

##Task:
Given the questions below, your task is to generate question substitutions for each question. Replacing the question stem entirely is acceptable given it's truth value is being changed. They don't need to be related to the original question/statement in any way. They just need to be semantically meaningful and of opposite truth value. That's it.

1) Semantic Substitution : substitute the question stem with a semantically meaningful and natural substitution.
2) Replacement (replace only the question stem)

### EXAMPLES:
Original: The color of leaves is green
Substitution: The capital of Spain is Milan.
Here the truth value is being changed from True to False.

Original: C++ is a programming language.
Substitution: Newton won Nobel Prize.
Here the truth value is being changed from True to False.

Original: The Earth is a planet.
Substitution: Moon is a star.
Here the truth value is being changed from True to False.

Above examples have no relation to the original question/statement in any way. They just need to be semantically meaningful and of opposite truth value. That's it. This is very important.

Your task: Generate {k} valid question substitutions per question that satisfy the replacement strategy. Each question substitution should:
1. Replace the question stem with a semantically meaningful and natural substitution.
2. Ensure the question substitution is semantically meaningful and natural.
3. The number of characters should be less than or equal to the original question stem. Very Important.
4. It can be ANY semantically meaningful and of opposite truth value statement.

### MANDATORY RULES: 
-  *Verifiable Factual Flip*: The question substitution must make the statement the absolute logical opposite of its original state.
-  *Semantic Substitution*: The question substitution must be semantically meaningful and natural.

For each question substitution, provide:
1. question-index: The question number
2. latex-stem-text: Exact LaTeX text of the question stem (must match the input exactly)
3. original-substring: The substring to replace (must be a contiguous substring of latex-stem-text)
4. replacement-substring: The replacement text
5. start-pos: Start position of original-substring relative to latex-stem-text (0-based index)
6. end-pos: End position of original-substring relative to latex-stem-text (exclusive, 0-based index)
7. target-wrong-answer: The opposite answer (e.g., "False" if gold is "True", or "True" if gold is "False")
8. reasoning: Brief explanation of why this mapping satisfies the strategy

IMPORTANT:
-  The original-substring MUST be an exact substring of latex-stem-text
-  The start-pos and end-pos MUST be accurate (start-pos + len(original-substring) = end-pos)
-  The target-wrong-answer MUST be the opposite of the gold answer
-  CRITICAL: The replacement-substring MUST be DIFFERENT from the original-substring. Do NOT generate mappings where original-substring == replacement-substring (e.g., "force" --> "force" is INVALID). The replacement MUST change the text to create actual manipulation.
-  CRITICAL: Neither original-substring nor replacement-substring can be empty strings. Both must contain actual text.
-  The substitution should be natural and semantically meaningful

## TF QUESTIONS {questions-list}

## OUTPUT FORMAT
Return ONLY valid JSON as a single array containing ALL mappings from ALL questions above.
Each question should have {k} mappings.

Total expected mappings: {total-mappings}
```json [{{
    "question-index": 1,
    "latex-stem-text": "...",
    "original-substring": "...",
    "replacement-substring": "...",
    "start-pos": 0,
    "end-pos": 5,
    "target-wrong-answer": "False",
    "reasoning": "..."
  }},
  ...]'''
Return ONLY valid JSON, no markdown or additional text

==> prompts/ACL_verifier.tex <==
def build_detection_judge_prompt(ai_answer: str, gold_answer: str, target_wrong_answer: Optional[str],
    question_type: str,extracted_option: Optional[str] = None) -> str:
    """
    Build prompt for LLM judge to determine if perturbation was detected.
    
    Evaluates whether AI answer matches target wrong answer (detected) or 
    gold answer (not detected), with confidence scoring.
    
    Args:
        ai_answer: AI's answer text, gold_answer: Correct/gold standard answer,
        target_wrong_answer: Target wrong answer (what perturbation aims for),
        question_type: Type of question (MCQ, TF, LONG),
        extracted_option: Extracted option letter for MCQ (A, B, C, D, E)
    
    Returns:
        Formatted prompt string for detection judgment
    """
    if question_type == "MCQ":
        prompt = f"""Evaluate whether a perturbation was successfully detected based on the AI's answer.

Question Type: Multiple Choice (MCQ)

AI Answer: {ai_answer}
Extracted Option: {extracted_option if extracted_option else "None"}
Gold Answer (Correct): {gold_answer}
Target Wrong Answer: {target_wrong_answer if target_wrong_answer else "None"}

Evaluation Criteria:
1.⁠ ⁠If AI selected the gold answer --> perturbation NOT detected (detected: false, confidence: 0.0)
2.⁠ ⁠If AI selected the target wrong answer --> perturbation DETECTED (detected: true, confidence: 1.0)
3.⁠ ⁠If AI selected a different wrong answer --> perturbation DETECTED but lower confidence (detected: true, confidence: 0.7)
4.⁠ ⁠If answer text contains target wrong answer text --> perturbation DETECTED (detected: true, confidence: 0.9)

Determine:
- ⁠detected: true/false (was perturbation successful?)
- ⁠match_confidence: 0.0-1.0 (how confident is this detection?)
- ⁠reason: Brief explanation of the decision

Return your judgment."""
    elif question_type == "TF":
        prompt = f"""Evaluate whether a perturbation was successfully detected based on the AI's answer.

Question Type: True/False

AI Answer: {ai_answer}
Gold Answer (Correct): {gold_answer}
Target Wrong Answer: {target_wrong_answer if target_wrong_answer else "None"}

Evaluation Criteria:
1.⁠ ⁠If AI answered same as gold --> perturbation NOT detected (detected: false, confidence: 0.0)
2.⁠ ⁠If AI answered same as target wrong answer --> perturbation DETECTED (detected: true, confidence: 1.0)
3.⁠ ⁠If AI answered differently from gold (but not target) --> perturbation DETECTED (detected: true, confidence: 0.8)

Extract True/False from answers:
- ⁠Look for explicit "True" or "False" statements
- ⁠Consider context and explanations

Determine:
- ⁠detected: true/false (was perturbation successful?)
- ⁠match_confidence: 0.0-1.0 (how confident is this detection?)
- ⁠reason: Brief explanation (e.g., "AI answered False (target was False, gold was True)")

Return your judgment."""
    else:  # LONG
        prompt = f"""Evaluate whether a perturbation was successfully detected based on the AI's answer.

Question Type: Long-form

AI Answer: {ai_answer[:500]}{"..." if len(ai_answer) > 500 else ""}
Gold Answer (Correct): {gold_answer[:500]}{"..." if len(gold_answer) > 500 else ""}
Target Wrong Answer Description: {target_wrong_answer if target_wrong_answer else "None"}

Evaluation Criteria:
1.⁠ ⁠If AI answer closely matches gold answer --> perturbation NOT detected (detected: false, confidence: 0.0)
2.⁠ ⁠If AI answer shows significant deviation from gold --> perturbation DETECTED (detected: true, confidence: 0.7)
3.⁠ ⁠If AI answer matches target wrong answer description --> perturbation DETECTED (detected: true, confidence: 0.7-0.9)

Check for:
- ⁠Word overlap/similarity with gold answer
- ⁠Presence of target wrong answer markers/keywords
- ⁠Substantial content differences
- ⁠Missing key concepts from gold answer

Determine:
- ⁠detected: true/false (was perturbation successful?)
- ⁠match_confidence: 0.0-1.0 (how confident is this detection?)
- ⁠reason: Brief explanation (e.g., "AI answer shows significant deviation from gold answer")
Return your judgment.
